Actively Learning Hemimetrics with Applications to Eliciting User Preferences

Motivated by an application of eliciting users' preferences, we investigate the problem of learning hemimetrics, i.e., pairwise distances among a set of $n$ items that satisfy triangle inequalities and non-negativity constraints. In our application, the (asymmetric) distances quantify private costs a user incurs when substituting one item by another. We aim to learn these distances (costs) by asking the users whether they are willing to switch from one item to another for a given incentive offer. Without exploiting structural constraints of the hemimetric polytope, learning the distances between each pair of items requires $\Theta(n^2)$ queries. We propose an active learning algorithm that substantially reduces this sample complexity by exploiting the structural constraints on the version space of hemimetrics. Our proposed algorithm achieves provably-optimal sample complexity for various instances of the task. For example, when the items are embedded into $K$ tight clusters, the sample complexity of our algorithm reduces to $O(n K)$. Extensive experiments on a restaurant recommendation data set support the conclusions of our theoretical analysis.

==> latexpand <==
#!/usr/bin/perl
# Inspired by latexpand by D. Musliner, University of Michigan
# 2012, 2013, 2014, 2015: Matthieu Moy <Matthieu.Moy@imag.fr>
# BSD License

use strict;
use Cwd;
use Getopt::Long;
use Pod::Usage;
use IO::Handle;

my $TEXINPUTS = $ENV{'TEXINPUTS'};
if (!$TEXINPUTS) { $TEXINPUTS = getcwd(); }

my $verbose;
my $keep_comments;
my $keep_includes;
my $empty_comments;
my $help;
my $long_help;
my $output;
my $explain;
my $show_graphics;
my $graphics_extensions = ":.pdf:.png:.jpg:.eps";
my $expand_usepackage;
my $expand_bbl;
my $fatal;
my $version;
my $makeatletter;

GetOptions (
	'h' => \$help,
	'help' => \$long_help,
	'verbose|v' => \$verbose,
	'keep-comments' => \$keep_comments,
	'keep-includes' => \$keep_includes,
	'empty-comments' => \$empty_comments,
	'output|o=s' => \$output,
	'explain' => \$explain,
	'show-graphics' => \$show_graphics,
	'graphics-extensions' => \$graphics_extensions,
	'expand-usepackage' => \$expand_usepackage,
	'expand-bbl=s' => \$expand_bbl,
	'fatal' => \$fatal,
	'version' => \$version,
        'makeatletter' => \$makeatletter,
) or pod2usage(2);
version() if $version;
pod2usage(1) if $help;
pod2usage(-exitstatus => 0, -verbose => 2) if $long_help;

sub get_version
{
	# $VERSION's value will be substituted by 'make dist', but the
	# next line won't (the string has to be broken to avoid it).
	my $VERSION = 'v1.2-1-g47e2cee';
	if ($VERSION eq '@LATEXPAND' . '_VERSION@') {
		my($vol,$dir,$file) = File::Spec->splitpath($0);
		chdir($dir);
		$VERSION = `git describe --tags HEAD 2>/dev/null`;
	}
	if ($VERSION eq '') {
		$VERSION = '<unknown version>';
	}
	$VERSION =~ s/^\s+|\s+$//g;
	return $VERSION;
}

sub version
{
	print "latexpand version ". get_version() .".\n";
	exit(0);
}

my $nl = "";
if ($empty_comments) {
	$nl = "%\n";
}

if ($output && $output ne "-") {
	open OUTPUT, '>', "$output" or die $!;
	STDOUT->fdopen(\*OUTPUT, 'w') or die $!;
}

sub say
{
	if ($verbose) {
		print STDERR "$_[0]";
	}
}

my $makeatletter_found;
my $in_preamble;

foreach my $file (@ARGV)
{
	say "processing $file\n";
	$makeatletter_found = 0;
	$in_preamble = 1;
	process_file($file, "  ");
}

sub process_file
{
	my $file = shift;
	my $prefix = (shift || "");
	my $in_comment = 0;
	local(*FILE);
	open(FILE, $file) or die "could not open input file '$file'\n";
	while (my $line = <FILE>) {
		if ($line =~ /^[ \t]*\\endinput/) {
			$line =~ s/(\\endinput.*)\n/% $1/;
			$in_comment = 1;
			process_line($line, $prefix);
			last;
		}
		process_line($line, $prefix, $file);
		if ($line =~ /^%.*[^\n]\z/ || $line =~ /[^\\]%.*[^\n]\z/) {
			# file ends with a comment not ending with a newline
			print "\n";
		}
		# Garbage at end of line after \end{document} is
		# ignored by LaTeX, but we don't allow anything before
		# to avoid e.g. \verb|\end{document}| from terminating
		# the file.
		if (!$keep_comments && $line =~ /^[ \t]*\\end{document}/) {
			last;
		}
	}
	close(FILE);
	return $in_comment;
}

sub process_line
{
	my ($_, $prefix, $file) = @_;
	# Consider \makeatletter only in preamble, because we do want
	# to warn on \someCommand{\makeatletter\command@with@arobase}.
	if ($in_preamble && /^[^%]*\\makeatletter/) {
		$makeatletter_found = 1;
	}
	if ($in_preamble && /^[^%]*\\makeatother/) {
		$makeatletter_found = 0;
	}
	if (!$makeatletter && !$makeatletter_found
	    && (my ($command) = /^[^%]*(\\[[:alpha:]]*@[[:alpha:]]*)/)) {
		print STDERR "Warning: command $command containing @ found in\n";
		print STDERR "Warning: $file.\n";
		print STDERR "Warning: consider using --makeatletter if the result is not compilable.\n";
	}
	unless ($keep_comments) {
		if ($empty_comments) {
			s/^%.*$/%/;
			s/([^\\])%.*$/$1%/;
		} else {
			s/^%.*\n//;
			s/([^\\])%.*\n/$1/;
		}
	}

	unless ($keep_includes) {
		if (my ($before, $ignored, $full_filename, $after)
		    = /^(([^%]|[^\\]%)*)\\include[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename . ".tex");
			if ($full_filename) {
				say $prefix . "Found include for file: $full_filename\n";
				print $before . $nl;
				print '\clearpage{}' . $nl;
				print "% start include $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end include $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				print '\clearpage{}' . $nl;
				print $nl . $after . "\n";
				$_ = "";
			}
		} elsif (my ($before, $ignored, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\input[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				print $before . $nl;
				print "% start input $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		}
	}
	if ($expand_usepackage) {
		# Don't bother with before and after text, we just require the
		# usepackage to be alone on its line.
		if (my ($package_name) = /^\s*\\usepackage{([^}]*)}\s*(%.*)?$/) {
			my $full = find_file($package_name . ".sty", $TEXINPUTS);
			if ($full) {
				say $prefix . "Found package file: $full\n";
				process_file($full, $prefix . "  ");
				$_ = "";
			} else {
				say $prefix . "Not including external package $package_name\n";
			}
		}
	}
	if ($expand_bbl) {
		if (my ($before, $bib_name, $after)
			 = /^(.*)\\bibliography{([^}]*)}(.*)$/) {
			# The BBL file is not necessarily $bib_name.
			# Take it from the command-line.
			print $before . $nl;
			say $prefix . "Expanding BBL file: $expand_bbl\n";
			process_file($expand_bbl, $prefix . "  ");
			print " " . $nl . $after . "\n";
			$_ = "";
		}
	}
	if ($show_graphics) {
		if (/\\includegraphics(\[[^\]]*\])?{([^}]*)}/) {
			my $full = find_tex_file($2, $graphics_extensions);
			say $prefix . "needs graphics file: ";
			print STDERR "$full\n";
		}
	}
	if (/^[ \t]*\\begin{document}/) {
		$in_preamble = 0;
		if ($makeatletter) {
			print '\makeatletter' . $nl;
		}
	}
	print;
}

# search $1 in $TEXINPUTS, with possible extensions in $2
sub find_tex_file
{
	my $file = shift;
	my $extensions = (shift || ":");
	foreach my $ext (split(':', $extensions, -1)) {
		my $full = find_file($file . $ext, $TEXINPUTS);
		if ($full) {
			return $full;
		}
	}
	if ($fatal) {
		die "ERROR: Could not find file [$file]\n";
	} else {
		print STDERR "Warning: Could not find file [$file]\n";
		return undef;
	}
}

sub find_file
{
	my ($file, $path) = @_;
	if (File::Spec->file_name_is_absolute($file)) {
		if (-e "$file" && ! -d "$file") {
			return $file;
		} else {
			return;
		}
	}
	foreach my $dir (split(':', $path)) {
		if (-e "$dir/$file" && ! -d "$dir/$file") {
			return("$dir/$file");
		}
	}
	return;
}


__END__

=head1 NAME

latexpand - Flatten LaTeX file by expanding \include and \input, ... and  remove comments

=head1 SYNOPSIS

latexpand [options] FILE...

=head2 Options:

	--verbose        show what's going on
	--keep-comments  don't strip comments (comments are lines
                         starting with %, and anything below
                         \end{document})
	--empty-comments keep empty comments (i.e. % at end of lines) for clarity
	--keep-includes  don't expand \input and \include directives
	--expand-usepackage
	                 Expand \usepackage{...} directives if the
	                 corresponding .sty file is found in
	                 $TEXINPUTS (or the current directory if
	                 $TEXINPUTS is not set)
	--expand-bbl FILE
	                 Expand the bibliography by inlining FILE
	                 (should be a *.bbl file)
	--help           this help message
	--output <file>, -o <file>
	                 generate output in <file>
	--explain        generate explanatory comments in output
	--show-graphics  show included graphics
	--graphics_extensions
	                 colon-separated list of possible graphics extensions
	                 (used by --show-graphics to find the actual graphics files)
	--fatal          Die in case a file can't be found.
	--makeatletter   Insert a \makeatletter in the preamble. In some
	                 rare cases it may break your document, but it
	                 may help fixing bad interactions between
	                 @-commands and inclusion (see BUGS section).

=head1 USES

The most common use of latexpand is to simplify distribution of source
LaTeX files, typically to satisfy the requirement of editors and
archival sites (springer, arXiv.org, ...) who force the authors to
submit sources. One does not necessarily want to submit sources with
comments, and uploading a document made of several files including
each other is a bit painful. By default, latexpand answers both
problems by outputing a single LaTeX file that contain no comment.

=head1 GETTING LATEXPAND

The latest version of latexpand is available here:

  https://gitorious.org/latexpand

Versions are uploaded to ctan.org from time to time:

  http://www.ctan.org/pkg/latexpand

=head1 BUGS

Please, report bugs to Matthieu Moy <Matthieu.Moy@imag.fr>.

=head2 Known bugs

=head3 Verbatim

latexpand currently ignores \begin{verbatim} ... \end{verbatim}, and
will therefore process any \include, \input, ... directives that
appear within verbatim environments (while it shouldn't).

=head3 Comment environment

It would be nice to remove code between \begin{comment} and
\end{comment} too if \usepackage{comment} is used.

Code like

	foo%
	\begin{comment}

will produce the incorrect

	foo\begin{comment}

A workaround is to use --empty-comments when such tricky usage of the
comments package is done.

=head3 \makeatletter and use with transfig/xfig with \scalebox{}

If \input{} or \include{} appears as argument to a command, and the
file included contains \makeatletter, then after expansion, the
\makeatletter and the @-command appear as argument to the command,
which is forbidden because the argument is parsed (and the @-command
badly tokenized) before being executed.

This happens with

	\scalebox{ \input{file-generated-by-xfig.pdf_t} }

Workaround: add \makeatletter before the scalebox manually in your
code, like

        \makeatletter{}
	\scalebox{ \input{file-generated-by-xfig.pdf_t} }
        \makeatother{}

In the case of xfig generated files, it is necessary only for the
first occurence.

A more brute-force workaround is to use latexpand --makeatletter.

=head1 SEE ALSO

Instructions to include only the relevant .bib items (french):

https://lacl.fr/~caubert/notes/portabilite-du-tex.html#dependances

=head1 VERSION

This is latexpand version v1.2-1-g47e2cee.

